SigSpec User's Manual

{\sc SigSpec} computes the spectral significance levels for the DFT amplitude spectrum of a time series at arbitrarily given sampling. It is based on the analytical solution for the Probability Density Function (PDF) of an amplitude level, including dependencies on frequency and phase and referring to white noise. Using a time series dataset as input, an iterative procedure including step-by-step prewhitening of the most significant signal components and MultiSine least-squares fitting is provided to determine a whole set of signal components, which makes the program a powerful tool for multi-frequency analysis. Instead of the step-by-step prewhitening of the most significant peaks, the program is also able to take into account several steps of the prewhitening sequence simultaneously and check for the combination associated to a minimum residual scatter. This option is designed to overcome the aliasing problem caused by periodic time gaps in the dataset. {\sc SigSpec} can detect non-sinusoidal periodicities in a dataset by simultaneously taking into account a fundamental frequency plus a set of harmonics. Time-resolved spectral significance analysis using a set of intervals of the time series is supported to investigate the development of eigenfrequencies over the observation time. Furthermore, an extension is available to perform the {\sc SigSpec} analysis for multiple time series input files at once. In this MultiFile mode, time series may be tagged as target and comparison data. Based on this selection, {\sc SigSpec} is capable of determining differential significance spectra for the target datasets with respect to coincidences in the comparison spectra. A built-in simulator to generate and superpose a variety of sinusoids and trends as well as different types of noise completes the software package at the present stage of development.

==> CoAst_layo.tex <==
\pagestyle{fancyplain}
\addtolength{\headwidth}{\marginparsep}
\addtolength{\headwidth}{\marginparwidth}
\addtolength{\headwidth}{\marginparwidth}
\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
\renewcommand{\sectionmark}[1]{\markright{#1}}
\lhead[\fancyplain{}{\sffamily\thepage}]{\fancyplain{}{\sffamily}}
\rhead[\fancyplain{}{\sffamily\leftmark}]{\fancyplain{}{\sffamily\thepage}}
%\rfoot[]{\fancyplain{}{\sffamily\small Communications in Asteroseismology, No. 131, July 2001}}
%\lfoot[\fancyplain{}{\sffamily\small Communications in Asteroseismology, No. 131, July 2001}]{}
\cfoot{}
%\paperheight=230mm
%\paperwidth=150mm
\hoffset=-1cm
\voffset=1mm
\topmargin=-12mm
\headheight=5mm
\headwidth=115mm
\headsep=7mm
\oddsidemargin=1mm
\evensidemargin=1mm
\marginparwidth=0cm
\marginparsep=0cm
\renewcommand{\headrulewidth}{0pt}
\textwidth=115mm
\textheight=165mm
\footskip=10mm
\newcommand{\apj}{ApJ}
\newcommand{\aj}{AJ}  %************Stimmts?
\newcommand{\aap}{A\&A}  %*************Stimmts?
\newcommand{\mnras}{MNRAS}
\newcommand{\tspace}{\hspace{1.2em}}
\newcommand{\feh}{$[Fe/H]$}
\newcommand{\by}{\ensuremath{(b-y)}}       % b-y index
\newcommand{\nr}{\multicolumn{-1}{c}{\ensuremath{\lesssim 25}}}
\newcommand{\dss}{$\delta$~Scuti stars}                     % Style for Delta Scuti Stars (plur.)
\newcommand{\ds}{$\delta$~Scuti star}
\newcommand{\ngc}[1]{NGC~{#1}}                              % Style for NGCxxxx
\newcommand{\templogg}{\texttt{templogg}}                   % Style for "templogg" program name
\newcommand{\teff}{\ensuremath{T_{eff}}}             % T_eff
\newcommand{\logg}{\ensuremath{\log g}}                     % log g
\newcommand{\vsini}{\ensuremath{v\sin i}}                   % v sin 
\newcommand{\halpha}{H$\alpha$}  % H alpha
\def\kms {km~s$^{-1}$}
\def\kmss {km~s$^{-1}$~}
\def\cd {d$^{-1}$}

\newcommand{\kopf}{\small\itshape Comm. in Asteroseismology\\ 2008, in preparation}
\newcommand{\Authors}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\authors}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\Author}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\renewcommand{\author}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\Address}[1]{\begin{center}\small\sf #1 \end{center}}
\newcommand{\address}[1]{\begin{center}\small\sf #1 \end{center}}
\renewenvironment{abstract}{\section*{Abstract}\normalsize\sf}{}
\newcommand{\References}[1]{\begin{flushleft}{\large References\\}\vspace*{2mm}\small #1 \end{flushleft}}
%\newcommand{\references}[1]{\begin{flushleft}{\large References\\}\vspace*{2mm}\small #1 \end{flushleft}}

\newcommand{\chapterDSSN}[2]{\chapter[\sf\normalsize #1\\ \footnotesize \hspace*{5mm}by #2 \sf\normalsize][]{#1\\}\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\headDSSN}[2]{\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\chapterdssn}[2]{\chapter[\sf\normalsize #1\\ \footnotesize \hspace*{5mm}by #2 \sf\normalsize][]{#1\\}\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\headdssn}[2]{\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\figureDSSN}[5]{\begin{figure}[#4]
\centering
\includegraphics*[#5]{#1}
\caption{#2}
\label{#3}
\end{figure}}
\newcommand{\figuredssn}[5]{\begin{figure}[#4]
\centering
\includegraphics*[#5]{#1}
\caption{#2}
\label{#3}
\end{figure}}
\newcommand {\strich} {\begin{center} \vspace{0.5cm} \rule{1.5cm}{0.3mm} \end{center}}
\renewcommand{\chaptername}{}
\newcommand{\acknowledgments}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\acknowledgements}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\Acknowledgments}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\Acknowledgements}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}


==> caput_coast.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge CoAst  \\ Announcements \\
\end{center}



==> caput_editorialcomment.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}



\section*{Editorial statement for the following paper (entitled \\ {\it MOST found evidence for solar-type oscillations in the K2 giant star HD\,20884)} }
{\it \small The main message of the following paper is to report the detection of nonradial pulsation in a K giant. This is an important and controversial topic.

A key issue for this investigation is the reliability of the extracted frequencies. Your editor has spent his life with Fourier amplitude spectra of high-precision ground-based photometry. From that experience, Figure 3 of the paper
represents the natural result of instrumental instabilities and atmospheric transparency changes and does not deserve a second look. However, these are satellite observations without the typical ground-based difficulties -- but there may be different problems.

The statistical analyses can only help us in a limited way. It does not matter much whether one applies my favorite criterion of amplitude signal/noise ratio < 4, the SigSpec values, or another method. All these statistical analyses rely on assumptions of the nature of noise present in the data. Again, in ground-based photometry, we have found that the statistics are not reliable for low-frequency peaks. The obvious method to verify that certain peaks are not noise is to look at a comparison sample: the authors provide the results for another star with a simpler light curve. In my opinion, the issue is not yet solved.\normalsize}




==> caput_helas.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge HELAS  \\ News \\
\end{center}



==> caput_papers.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 


\newpage 

\pagenumbering{arabic}%
\setcounter{page}{1}%
%von mir geändert von 0 auf 1

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge Scientific  \\ Papers \\
\end{center}


\newcounter{paper} 
\stepcounter{paper}
\def\code{P}
%\renewcommand\thepage {\code\arabic{paper}-\arabic{page} } 

%\newcounter{paperpage}
%\stepcoutner{paperpage}{page}
%\thepage


%\stepcounter{paper}

%\newcommand\thepapercode{\code\thepaper-\thepage}

